Non-smooth Variable Projection

Variable projection solves structured optimization problems by completely minimizing over a subset of the variables while iterating over the remaining variables. Over the last 30 years, the technique has been widely used, with empirical and theoretical results demonstrating both greater efficacy and greater stability compared to competing approaches. Classic examples have exploited closed-form projections and smoothness of the objective function. We extend the approach to problems that include non-smooth terms, and where the projection subproblems can only be solved inexactly by iterative methods. We propose an inexact adaptive algonrithm for solving such problems and analyze its computational complexity. Finally, we show how the theory can be used to design methods for selected problems occurring frequently in machine-learning and inverse problems.

==> myhead.tex <==
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{graphicx}

\newcommand{\argmax}{\operatornamewithlimits{arg max}}
\newcommand{\argmin}{\operatornamewithlimits{arg min}}
\newcommand{\prox}{\operatornamewithlimits{prox}}

\usepackage{algorithm}
\usepackage{algpseudocode}

\newcommand{\RR}{\mathbb{R}}
\newcommand{\dist}{\textrm{dist}}
%
\newtheorem{thm}{Theorem}
\newtheorem{corollary}{Corollary}

\newcommand{\ts}[1]{{\textstyle#1}}
% \usepackage{microtype}
% %\usepackage{units}
% \usepackage{amsmath}
% \usepackage{amsthm}
% \usepackage{amssymb}
% \usepackage{mathtools}
% \usepackage[margin=1in]{geometry}
% \usepackage{color}
% \usepackage{url}
% \usepackage{multicol}
% \usepackage{hyperref}
% \usepackage{graphicx}
% \usepackage{caption}
% \usepackage{subcaption}
% \usepackage{cite}
% \usepackage{booktabs}
% %\usepackage{pgfplots}\pgfplotsset{compat=1.4}
% %\usepackage{subdepth}
% %\usepackage{refcheck}
%
% \usepackage{amsfonts}
% %\usepackage{epsfig}
% %\usepackage{graphicx}
% %\usepackage{multicol}
% %\usepackage{color}
% %\usepackage{crop}
% %%\usepackage{natbib}
% %\usepackage{float}
% %\usepackage{booktabs}
% %usepackage{algorithmic}
% %\usepackage{algorithm}
% %\usepackage{hyperref}
% %\usepackage[autolinebreaks,useliterate]{mcode}
% %%\usepackage{pstricks}
% %% Sasha's macros:
%
% \newcommand{\B}[1]{{\bf #1}}
% \newcommand{\R}[1]{{\rm #1}}
% \newcommand{\Sc}[1]{{\mathcal{#1}}}
% %\newtheorem{remark}{Remark}[section]
% %\newtheorem{theorem}{Theorem}[section]
% %\newtheorem{corollary}{Corollary}[section]
% %\newtheorem{lemma}{Lemma}[section]
%
% %\newenvironment{proof}[1][Proof]{\begin{trivlist}
% %\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
% %\newcommand{\FF}{{\mathcal{F}}}
% %\newcommand{\rank}{{\rm rank}}
% \newcommand{\trace}{\mathsf{trace}}
% \newcommand{\vect}{\mathsf{vec}}
% \newcommand{\stackt}{\mathsf{stack}}
% \newcommand{\dictt}{\mathsf{dictionary}}
% \newcommand{\blkdt}{\mathsf{blockdiag}}
%
% \newcommand{\mbf}[1]{\mathbf{#1}}
% \newcommand{\mcl}[1]{\mathcal{#1}}
% \newcommand{\msf}[1]{\mathsf{#1}}
% \newcommand{\transp}[1]{{#1}^{*}}
% \newcommand{\argmax}{\operatornamewithlimits{arg max}}
% \newcommand{\argmin}{\operatornamewithlimits{arg min}}
% \newcommand{\prox}{\operatornamewithlimits{prox}}
% \newcommand{\ts}[1]{{\textstyle#1}}
% \newcommand{\ds}[1]{{\displaystyle#1}}
% \newcommand{\bq}{\begin{eqnarray}}
% \newcommand{\eq}{\end{eqnarray}}
% \newcommand{\todo}[1]{\begin{center}{\color{red} TODO:} \emph{#1}\end{center}}
% %\renewcommand{\eqref}[1]{equation (\ref{eq:#1})}
% \newcommand{\Eqref}[1]{Equation (\ref{eq:#1})}
% \newcommand{\figref}[1]{figure \ref{fig:#1}}
% \newcommand{\Figref}[1]{Figure \ref{fig:#1}}
% \newcommand{\intd}[1]{\int\!\!\mathrm{d}#1}
% \newcommand{\intdl}[3]{\int_{#2}^{#3}\!\!\mathrm{d}#1}
% \newcommand{\mbfs}[1]{\mbox{\boldmath$#1$}}
% \newcommand{\sinc}{\mathrm{sinc}}
% \newcommand{\sgn}{\operatorname{{\mathrm sgn}}}
% %\newcommand{\qed}{\nobreak \ifvmode \relax \else
% %      \ifdim\lastskip<1.5em \hskip-\lastskip
% %      \hskip1.5em plus0em minus0.5em \fi \nobreak
% %      \vrule height0.75em width0.5em depth0.25em\fi}
% \renewcommand{\Pi}{\mbox{\LARGE$\pi$}}
% %\newcommand{\WF}{\operatorname{{\mathrm WF}}}
% %\newcommand{\diag}{\mathrm{diag}}
%
% %\renewcommand{\algorithmiccomment}[1]{// #1}
% % \newtheorem{theorem}{Theorem}[section]
% % \newtheorem{lemma}[theorem]{Lemma}
% % \newtheorem{proposition}[theorem]{Proposition}
% % \newtheorem{corollary}[theorem]{Corollary}
% %
%
% \newcommand{\am}{\operatornamewithlimits{argmin}}
% \newcommand{\amm}{\operatornamewithlimits{argmax}}
%
%
% % \newenvironment{proof}[1][Proof]{\begin{trivlist}
% % \item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
% %\newenvironment{definition}[1][Definition]{\begin{trivlist}
% %\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
% % \newenvironment{example}[1][Example]{\begin{trivlist}
% % \item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
% %\newenvironment{remark}[1][Remark]{\begin{trivlist}
% % \item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%
% %\definecolor{MyGray}{rgb}{0.96,0.97,0.98}
%
% %\makeatletter\newenvironment{graybox}{%
% %   \begin{lrbox}{\@tempboxa}\begin{minipage}{.9\columnwidth}}{\end{minipage}\end{lrbox}%
% %   \colorbox{MyGray}{\usebox{\@tempboxa}}
% %}\makeatother
% \newcommand{\RR}{\mathbb{R}}
% \newcommand{\dist}{\textrm{dist}}
%
% \newtheorem{thm}{Theorem}
% \newtheorem{cor}{Corollary}
% \newtheorem{algo}{Algorithm}
% \newtheorem{corollary}{Corollary}
%
% %
% \usepackage[noend]{algpseudocode}
% \usepackage{algorithm}
% \usepackage{algorithmic}
% % \newcommand*\Let[2]{\State #1 $\gets$ #2}
% \algrenewcommand\algorithmicrequire{\textbf{Input:}}
% \algrenewcommand\algorithmicensure{\textbf{Output:}}
% % %\resetcounteronoverlays{algorithm}
% %
% % \usepackage{color}
% % \newcommand{\red}[1]{\textcolor{red}{#1}}


==> survey.tex <==
\section{Nonsmooth Variable Projection in Applications \label{sec:survey}}


%As alluded to in the introduction, the variable projection technique has been widely used in different application domains.
In this section, we describe three applications where nonsmooth VP plays a role: exponential data fitting, robust inference, and multiple kernel learning. %, and PDE-constrained optimization.
%Despite the variety of these applications, the underlying algorithmic techniques all fall within the same paradigm.
%However, there are subtle modifications that may be required to make the scheme work, which we emphasize when appropriate.
%We begin with ODE or PDE constrained problems.

%[CAN WE SAY SOME MORE STUFF HERE? SOMETHING LIKE: WHILE FOR MANY APPLICATIONS A LOT THEORY AND EFFICIENT APPROACHES EXISTS (ADJOINT STATE) WHILE FOR OTHERS THE VP FORMALISM SHEDS NEW LIGHT BLABLA..]

% the paper already sounds like "while a lot of practical practitioners design algorithmic methods based on insufficient theory, their efficacy only undergirds the importance of the luminance of the VP formalism on
% subtle distinctions that we endeavor to emphasize".




%\paragraph{Direction-of-Arrival estimation}
%We want to measure the direction of incoming plane waves measured by an array of antennas.
%The signal model is
%\[
%{y} = \sum_{k=1}^{M} a_i\exp(\imath k_i {x}),
%\]
%where ${x} = [0, h, \ldots, (N-1)h]$ encodes the array. Introducing the matrix $A({k})$
%with elements  $a_{ij} = \exp(\imath k_jx_i)$, we write the noisy measurements as
%\[
%{y} = A({k}){a} + {n}.
%\]
%A natural approach is to formulate a nonlinear least squares problem,
%\[
%\min_{{a},{k}} \|A({k}){a} - {y}\|_2^2,
%\]
%which is readily solved using the variable projection algorithm. In practice, however, we don't know the number of parameters, $M$, to include. We can over-parametrize the problem, choosing a rather large value for $M$, but this may lead to unreliable estimates. By including a sparsity prior on ${a}$ we force the optimization to find a solution with the least possible amount of parameters.
%We can now pose the problem as follows
%\[
%\min_{{a},{k}} \|A({k}){a} - {y}\|_2^2 + \lambda\|{a}\|_1.
%\]
%Note also that we can replace the $\ell_2$ data misfit term to account
%for the statistics of the noise. The variable projection approach allows us to efficiently solve this problem by projecting out ${a}$ using any suitable method to solve LASSO problems and using a non-linear optimization method to find the optimal ${a}$.
%
%In our numerical experiments, we show the utility of this approach compared to conventional DOA estimation. We also show
%that variable projection works much better in practice than approaches that iterate in the full space of  ${a},{k}$.
%

%\paragraph{Parametric blind deconvolution}
%A similar problem to direction of arrivals estimation is to decompose a given noisy image into a set of (parametrized) basis functions.
%The image can be written as
%\begin{equation}
%{y} = \sum_{i=1}^{M}a_{i}\phi(({x} - {c}_i)/r_i),
%\end{equation}
%where the number of terms $M$, the locations ${c}_i$, the scales $r_i$ and the amplitude $a_i$ are positive and unknown. Analogously to DOA, we do not know the number of signals we wish to use; and so we formulate a nonsmooth variable projection problem,
%using sparsity to eliminate unnecessary signals.
%\begin{equation}
%\min_{{a}\geq 0, {c}, {r}} \|A({c},{r}){a} - {y} \|_2^2 + \lambda \|{a} \|_1.
%\end{equation}
%
%In the numerical example, we show the advantage of the projected approach, using basis functions $\phi(\cdot) = \exp(-\|\cdot\|^2)$.
%An interesting extension here is the non-negativity constraint on the $a$ parameters.



Introducing the matrix $\Phi(x)$ with entries $\Phi(x)_{ij}:=\exp(-\varphi_{ij}(x))$, we express the noisy measurements as
\[
{y} = \Phi(x){\theta} + {\epsilon}.
\]
A natural approach is then to formulate a nonlinear least squares problem,
\[
\min_{{\theta},{x}}~ \|\Phi(x){\theta} - {y}\|_2^2,
\]
which is readily solved using the classic VP algorithm.
In practice, however, we may not know the number of terms, $n$, to include.
We can over-parametrize the problem, choosing a large value for $n$, but this may lead to unreliable estimates and poor generelizability.
By including a sparsity-inducing prior on ${\theta}$ we force a more parsimonious solution:
\[
\min_{{\theta},{x}}~ \|\Phi(x){\theta} - {y}\|_2^2 + \lambda\|{\theta}\|_1.
\]
Additional constraints on $\theta$ may be added \citep{OLeary2012,Shearer2013}. Moreover, depending on the properties of the noise $\epsilon$ we may wish to impose a different on the residual.
%The variable projection approach allows us to efficiently solve this problem by projecting out ${\theta}$ using any suitable method to solve LASSO problems (we use IPsolve \citep{JMLR:aravkin13a}) and using a non-linear optimization method to find the optimal ${x}$.
%Indeed, we will see in Section~\ref{sec:theory} that provided  $\Phi(\theta)$ has full column rank for all $\theta$,
%the function
%\begin{equation}\label{eqn:vp_nonsm}
%\widetilde{f}(\theta)=\min_{a} f(\theta,a):=\|\Phi(\theta)a-y\|^2_2+\lambda\|a\|_1,
%\end{equation}
%is differentiable
%with gradient
%$\nabla \widetilde{f}(\theta)=\nabla_{\theta}  f(\theta,\bar{a})$ where $\bar{a}$ achieves the minimum.

This leads us to consider the joint problem
\begin{equation}
\label{eq:VPgen}
\min_{{\theta},{x}} f(x,\theta) := \rho(\Phi(x){\theta} - {y}) + R(\theta)
\end{equation}
with $\rho$ convex and smooth, and $R$ convex and nonsmooth (e.g. 1-norm) and potentially infinite
valued (e.g. infinity off of a box).

We develop an inexact gradient algorithm, using an iterative method on the inner problem in $\theta$
to obtain gradient estimates of the outer problem, with controlled errors.
When $\Phi$ has full column rank, and $R$ admits a proximity operator,
proximal gradient methods converge at a {\it linear rate} on the $\theta$ sub-problem,
so each inner problem requires virtually the same number of iterations as we tighten the error tolerance.
If $\Phi(x)$ does not have full column rank, we can add a quadratic regularizer in $\theta$ (replacing the 1-norm with the elastic net), and obtain an analogous result. The new approach is more effective and stable than joint first-order optimization in $(\theta, x)$, see section~\ref{sec:num_ill}.





%\subsection{PDE-constrained optimization}
%Physical systems often give rise to optimization problems with ODE and PDE constraints; see e.g. optimal control \citep{Dennis1998,Philip2009} and inverse problems in geophysics \citep{Haber2000,Biros} astrophysics \citep{Hanasoge2014} and medical imaging \citep{Abdoulaev2005}. Setting notation, consider the problem
%\begin{equation} %\label{eq:NLP}
%\label{eq:class}
%\min_{x,u}~ g(x,u) \quad \mbox{s.t.} \quad c(x,u) = 0,
%\end{equation}
%  where $u$ is the \emph{state} variable (a vector field), the system $c(x,u)=0$ is an ODE or PDE with parameters of interest $x$, and $g$ is an objective that we aim to minimize (e.g. data misfit). Here we assume that $g$ is lower bounded and convex. Upon discretization, $u$ becomes a high-dimensional vector. For the current exposition, we will assume that the PDE is linear. Abusing notation slightly, we assume that the system  \eqref{eq:class} is already discretized, and is in the form
%  \begin{equation} %\label{eq:NLP}
%  \label{eq:classPDE}
%  \min_{x,u}~ g(x,u) \quad \mbox{s.t.} \quad H(x)u = q,
%  \end{equation}
%  where $H(x)$ is a square invertible matrix depending $C^1$-smoothly on $x$, the function $g$ is $C^1$-smooth and the margin function $g(x,\cdot)$  is convex for each $x$. %We will denote the $i$'th column of $H(x)$ by the symbol $H_{i}(x)$.
%
%
%In large-scale applications, it is impractical to store and update the entire vector $u$. Instead, {\it adjoint state methods} compute $u$ on the fly and optimize in $x$ alone. Observe that the problem is equivalent to minimizing the smooth function
%$\widetilde f(x):=g(x,H(x)^{-1}q)$ and it is well-known \citep{Haber2000,plessix06} that $\nabla\widetilde f(x)$ is given by
%$$\nabla\widetilde{f}(x)=\nabla_x g(x,\bar u)+ \nabla \langle \bar{v}, H(\cdot)\bar{u}\rangle(x),$$
%where $(\bar u, \bar v)$ satisfy the equations
%\begin{equation}\label{eq:pdes}
%\left \{
%\begin{tabular}{rl}
%$H(x)^*\bar{v}+\nabla_u g(x,\bar u)$ &= 0 \\
%$H(x)\bar{u}$ &= $q$\\
%\end{tabular}
%\right \}.
%\end{equation}
%A variational viewpoint elucidates the formula. Indeed, basic convex duality (e.g. \cite[Corollary 3.3.11]{BL_book}) implies that $\widetilde{f}(x)$ can equivalently be written as
%\begin{equation}\label{eqn:var_proj}
%\widetilde{f}(x)=\sup_v \min_u~ g(x,u) + \langle v, H(x)u-q\rangle.
%\end{equation}
%%Although various derivations of the adjoint-state approach exist \citep{Haber2000,plessix06}, we present a short motivation based on the variable projection viewpoint.
%%To this end, observe that the formulation \eqref{eq:classPDE} is  equivalent to the problem
%%To do this we use an explicit representation of the indicator function of $0$:
%%\[
%%\delta_0(x) = \sup_{v} \langle v, x\rangle = \begin{cases} 0 & x = 0 \\ \infty & x \neq 0\end{cases}
%%\]
%%We can now rewrite~\eqref{eq:classPDE} as
%%\begin{equation}
%%\label{eq:classPDEexplicit}
%%\min_{x,u} \sup_v f(x, u, v) := g(x,u) + \langle v, H(x)u-q\rangle.
%%\end{equation}
%%Duality (e.g. \cite[Corollary 3.3.11]{BL_book}) implies that we can interchange $\min_u$ and $\sup_v$, yielding
%%\begin{equation}\label{eqn:var_proj}
%%\min_{x} \widetilde{f}(x):=\sup_v \min_u f(x, u, v).
%%\end{equation}
%%In section~\ref{sec:theory}, we will justify that $\widetilde{f}$ is differentiable, with the gradient having the following intuitive form.
%Now observe that equation \eqref{eq:pdes} simply says that $(\bar{u},\bar{v})$ is a saddle point of \eqref{eqn:var_proj} while the description of $\nabla\widetilde{f}(x)$ is the partial gradient with respect to $x$ of the inner function in \eqref{eqn:var_proj} evaluated at $(x,\bar u,\bar v)$.
%
%%denote the saddle point of \eqref{eqn:var_proj}, meaning
%%\[
%%\left\{
%% \begin{tabular}{rl}
%%\nabla_u g(x,\bar u)+H(x)^*\bar v&=0
%%H(x)\bar{u}&=q
%%\end{tabular}\right\}
%%\]
%%\[
%%\left \{
%%\begin{tabular}{rl}
%%$H(x)^*\bar{v}+\nabla_u g(x,\bar u)$ &= 0 \\
%%$H(x)\bar{u}$ &= $q$\\
%%\end{tabular}
%%\right \},
%%\]
%%the gradient $\nabla\widetilde{f}(x)$ is simply
%%$$\nabla\widetilde{f}(x)=\nabla_x \widetilde{f}(x,\bar u,\bar v)=\nabla_x g(x,\bar u)+ \nabla \langle \bar{v}, H(\cdot)\bar{u}\rangle(x).$$
%%immediately show that $\tilde{f}$ is differentiable with gradient
%%$$\nabla \tilde{f}(x)=\nabla_x g(\bar u,x)+ \sum_i \bar u_i\left(\nabla H_{i}(x)^*\bar v\right),$$
%%where  $\bar{u}$ is the unique solution of $H(x)u=q$ and $\bar{v}$ is the unique solution of the adjoint equation
%%$H(x)^* v + \nabla_u g(x,\overline u) = 0.$
%
%
%
%
%%
%%Now we can use variable projection to solve for both $\overline u$ and $\overline v$ to obtain a reduced objective
%%\begin{equation}
%%\widetilde{g}(x) = g(x,\overline u,\overline v),
%%\end{equation}
%%with gradient
%%\[
%%\nabla_x \widetilde{g}(x) = \nabla_x g(x,\overline u,\overline v) = \partial_x f(\overline u,x) + \partial_x \langle \overline v, c(x,\overline u) \rangle
%%= \partial_x f(\overline u ,x) + \langle \overline v, \partial_x c(x,\overline u) \rangle,
%%\]
%%with $\overline u$ being implicitly defined by $c(\overline u,x) = 0$, and $\overline v$ solving the adjoint equation
%%\[
%%\partial_u c(x,\overline{u})^*\overline v + \partial_u f(x,\overline u) = 0.
%%\]
%
%\paragraph{Penalty methods for PDE constrained optimization}
%%Note that in the least squares case $g(u,x)=\|Ru-d\|^2$,
%%the adjoint method requires two equation solves to compute $(\bar u, \bar v)$, in order to calculate the gradient $\nabla\widetilde f(x)$.
%In some applications, it may be desirable to relax the constraint $H(x)u=q$ and formulate a penalized problem introduced in \citep{vanLeeuwen2013Penalty2}
%\[
%\label{eq:penaltyPDE}
%\min_{x,u}~ g(u,x) + \lambda\cdot p\Big(H(x)u-q\Big),
%\]
%where $\lambda$ is a penalty parameter and $p$ is strongly convex, smooth penalty function (e.g. $p = {\textstyle\frac{1}{2}}\|\cdot\|_2^2$). The variable projection technique is immediate here.
%An easy application of \citep{RTRW}[Theorem 10.58]
%shows that the function
%\begin{equation}\label{eq:vp_penal}
%\widetilde g(x):=\min_u~ g(u,x)+\lambda \cdot p\Big(H(x)u-q\Big)
%\end{equation}
%is differentiable and its derivative is simply the partial derivative of the inner function in $x$ evaluated at $(x,\bar u)$,
%%$$\nabla \widetilde g(x)=\nabla_x g(\bar u,x)+\lambda\cdot \nabla H(x)^*\nabla p\Big(H(x)\bar u-q\Big),$$
% where $\bar u$ achieves the minimum. For an extended explanation, see Section~\ref{sec:theory}. Notice that in case of the least squares objective $g(u,x)=\|Ru-d\|^2$, only one equation solve is needed to compute $\bar u$ and hence the derivate $\nabla \widetilde g(x)$. This is in contrast to the adjoint method where another equation solve is needed to compute the adjoint variable $\bar v$. For promising numerical results, see  \citep{vanLeeuwen2013Penalty2}. Hence the variable projection technique, even in this rudimentary setting, can yield surprising computational benefits.
%
%%
%As with the adjoint-state formulation, we can project out the state variable $u$ and defined a reduced objective
%\[
%\widetilde{g}(x) = g(x,\overline u) + \lambda p(c(\overline u,x)),
%\]
%with $\overline u$ implicitly defined as the minimizer of $g(x,\cdot) + \lambda p(c(x,\cdot))$.

